SD-Track: Sparse-to-Dense Amodal Fusion for Question-Guided Tracking

Spatio-temporal video grounding (STVG) localizes objects in space and time from natural language queries, including direct descriptions and questions that require reasoning over video events. While recent zero-shot approaches use multimodal large language models (MLLMs) to guide visual tracking, trackers that propagate visible masks can underestimate an object's full extent under occlusion. We introduce SD-Track, a framework for amodal tracking that fuses sparse MLLM predictions with dense visual tracks. An MLLM identifies the queried objects and creates a shared tracking plan with instance identities, visibility intervals, and initial bounding boxes at reference frames. The plan guides a visual tracker to generate dense trajectories and the MLLM to estimate each object's full extent (amodal) at sparse frames. Our fusion combines SAM3's consistent tracking with Gemini's full extent estimation. It interpolates coordinate corrections from spatially consistent box pairs along dense tracks to account for occluded regions. SD-Track formed the basis of our winning solution in the Grounded VideoQA track of the Fourth Perception Test Challenge at ECCV 2026, where our team achieved first place with a HOTA score of 66.37. SD-Track achieves test-phase HOTA scores of 66.20 on Perception Test Grounded VideoQA and 13.31 on SVAG-Bench, outperforming the compared methods in HOTA. VidSTG results also show substantial improvements over the compared methods. Code and reproduction materials are available at https://github.com/BananaBats/2026-ECCV-Grounded-VQA.

==> sec/0_abstract.tex <==
\makeatletter
\let\qtrace@original@maketitle\@maketitle
\renewcommand{\@maketitle}{%
  \qtrace@original@maketitle
\begingroup
  \centering
  \includegraphics[width=\textwidth]{sec/figures/02_Full_sequence_all_three_methods.pdf}\par
  \captionsetup{hypcap=false}
  \captionof{figure}{\textbf{Complementary amodal and temporal cues in SD-Track.} Columns follow the same target cup through initialization, crossing, occlusion, and subsequent mixing. Rows compare sparse Gemini predictions (1 fps), dense SAM3 tracking (10 fps), and SD-Track. Under partial occlusion, SAM3’s visible-region box underestimates the target’s full extent (11.0 s). Gemini captures amodal extent but loses identity consistency when similar cups interact, selecting a different cup at 10.0 s and 16.0 s. SD-Track propagates reliable Gemini amodal corrections along dense SAM3 trajectories, recovering occluded extent while preserving target identity. Orange solid and blue dashed boxes denote predictions and ground truth, respectively.}
  \label{fig:qtrace-sequences}
\endgroup
  \vspace{6pt}%
}
\makeatother

\maketitle


% \begin{abstract}
% Spatio-temporal video grounding (STVG) localizes objects in space and time from natural language queries, including direct descriptions and questions that require reasoning over video events. While recent zero-shot approaches use multimodal large language models (MLLMs) to guide visual tracking, trackers that propagate visible masks can underestimate an object's full extent under occlusion. We introduce \textbf{SD-Track}, a framework for amodal tracking that fuses sparse MLLM predictions with dense visual tracks. An MLLM identifies the queried objects and creates a shared tracking plan with instance identities, visibility intervals, and initial bounding boxes at reference frames. The plan guides a visual tracker to generate dense trajectories and the MLLM to estimate each object's full extent (amodal) at sparse frames. Our fusion combines SAM3's consistent tracking with Gemini's full extent estimation. It interpolates coordinate corrections from spatially consistent box pairs along dense tracks to account for occluded regions. SD-Track achieves the highest test-phase HOTA on Perception Test Grounded VQA and SVAG-Bench, with scores of 66.20 and 13.31, respectively. VidSTG results also show substantial improvements over the compared methods.
% \end{abstract}

\begin{abstract}
Spatio-temporal video grounding (STVG) localizes objects in space and time from natural language queries, including direct descriptions and questions that require reasoning over video events. While recent zero-shot approaches use multimodal large language models (MLLMs) to guide visual tracking, trackers that propagate visible masks can underestimate an object's full extent under occlusion. We introduce \textbf{SD-Track}, a framework for amodal tracking that fuses sparse MLLM predictions with dense visual tracks. An MLLM identifies the queried objects and creates a shared tracking plan with instance identities, visibility intervals, and initial bounding boxes at reference frames. The plan guides a visual tracker to generate dense trajectories and the MLLM to estimate each object's full extent (amodal) at sparse frames. Our fusion combines SAM3's consistent tracking with Gemini's full extent estimation. It interpolates coordinate corrections from spatially consistent box pairs along dense tracks to account for occluded regions. SD-Track formed the basis of our winning solution in the Grounded VideoQA track of the Fourth Perception Test Challenge at ECCV 2026, where our team achieved first place with a HOTA score of 66.37. SD-Track achieves test-phase HOTA scores of 66.20 on Perception Test Grounded VideoQA and 13.31 on SVAG-Bench, outperforming the compared methods in HOTA. VidSTG results also show substantial improvements over the compared methods. Code and reproduction materials are available at \url{https://github.com/BananaBats/2026-ECCV-Grounded-VQA}.
\end{abstract}
